UniK3D: Universal Camera Monocular 3D Estimation

Monocular 3D estimation is crucial for visual perception. However, current methods fall short by relying on oversimplified assumptions, such as pinhole camera models or rectified images. These limitations severely restrict their general applicability, causing poor performance in real-world scenarios with fisheye or panoramic images and resulting in substantial context loss. To address this, we present UniK3D, the first generalizable method for monocular 3D estimation able to model any camera. Our method introduces a spherical 3D representation which allows for better disentanglement of camera and scene geometry and enables accurate metric 3D reconstruction for unconstrained camera models. Our camera component features a novel, model-independent representation of the pencil of rays, achieved through a learned superposition of spherical harmonics. We also introduce an angular loss, which, together with the camera module design, prevents the contraction of the 3D outputs for wide-view cameras. A comprehensive zero-shot evaluation on 13 diverse datasets demonstrates the state-of-the-art performance of UniK3D across 3D, depth, and camera metrics, with substantial gains in challenging large-field-of-view and panoramic settings, while maintaining top accuracy in conventional pinhole small-field-of-view domains. Code and models are available at github.com/lpiccinelli-eth/unik3d .

==> tables/ablations/ablations.tex <==
\begin{table*}[ht]
\centering
\caption{\textbf{Ablations.} \textit{Model} corresponds to the type of camera model employed, in particular, PH: pinhole, Leg: Legendre-polynomials (Spherical), Zer: Zernike-polynomials, NP: non-parametric. \textit{Data} indicates if images from strongly distorted cameras are used during training, either real or synthesized. \textit{Output} describes the predicted and supervised output space, either radial or the z-axis component, \ie depth. \textit{$\mathcal{L}_{\text{AA}}$} describes if the asymmetrical angular loss is employed, L1-loss otherwise. \textit{Cond} describes if the architecture and design changes described in \cref{ssec:method:engineer} are utilized.}
\label{tab:results:ablations}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccc|ccc|ccc|ccc|ccc}
\toprule
& \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Data}} & \multirow{2}{*}{\textbf{Output}} & \multirow{2}{*}{$\mathbf{\mathcal{L}}_{AA}$} & \multirow{2}{*}{\textbf{Cond}} & \multicolumn{3}{c|}{SFoV} & \multicolumn{3}{c|}{SFoV+Dist} & \multicolumn{3}{c|}{LFoV} & \multicolumn{3}{c}{Pano} \\
 & & & & & & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ \\
\midrule
1 & PH & \xmark & depth & \xmark & \xmark & $89.7$ & $55.1$ & $79.2$ & $91.8$ & $31.7$ & $60.0$ & $68.1$ & $41.2$ & $35.1$ & $32.5$ & $8.4$ & $4.2$ \\
2 & Leg & \xmark & depth & \xmark & \xmark & $90.2$ & $56.1$ & $79.1$ & $92.4$ & $34.5$ & $60.2$ & $71.9$ & $47.1$ & $56.7$ & $32.3$ & $11.3$ & $16.1$ \\
3 & PH & \cmark & depth & \xmark & \xmark & $88.9$ & $56.1$ & $81.1$ & $93.7$ & $40.4$ & $58.2$ & $70.1$ & $44.9$ & $43.1$ & $32.4$ & $5.9$ & $3.0$ \\
4 & Leg & \cmark & depth & \xmark & \xmark & $90.7$ & $56.2$ & $79.4$ & $94.4$ & $42.1$ & $62.7$ & $72.0$ & $48.5$ & $60.8$ & $32.6$ & $10.9$ & $14.8$ \\
5 & PH & \cmark & radius & \xmark & \xmark & $89.6$ & $56.0$ & $81.1$ & $93.2$ & $39.5$ & $57.6$ & $70.2$ & $44.4$ & $48.9$ & $35.4$ & $10.1$ & $4.9$ \\
6 & Leg & \cmark & radius & \xmark & \xmark & $89.6$ & $56.8$ & $76.7$ & $92.8$ & $35.0$ & $43.7$ & $78.7$ & $51.8$ & $61.1$ & $59.7$ & $53.8$ & $22.0$ \\
7 & Leg & \cmark & radius & \cmark & \xmark & $91.1$ & $57.7$ & $80.9$ & $94.2$ & $39.5$ & $52.1$ & $79.5$ & $52.9$ & $64.2$ & $57.6$ & $56.1$ & $24.4$ \\
8 & Leg & \cmark & radius & \cmark & \cmark & $90.5$ & $57.3$ & $79.8$ & $94.3$ & $44.6$ & $59.3$ & $81.2$ & $53.5$ & $64.8$ & $58.0$ & $58.6$ & $26.3$ \\
9 & Zer & \cmark & radius & \cmark & \cmark & $89.9$ & $56.6$ & $80.9$ & $93.5$ & $39.9$ & $51.3$ & $79.2$ & $49.9$ & $54.6$ & $52.8$ & $31.8$ & $17.9$ \\
10 & NP & \cmark & radius & \cmark & \cmark & $91.2$ & $56.4$ & $81.0$ & $93.9$ & $45.2$ & $62.8$ & $72.3$ & $42.0$ & $42.8$ & $53.2$ & $51.7$ & $20.1$ \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/ablations_2.tex <==
\begin{table*}[ht]
\centering
\caption{Ablations Contd}
\label{tab:results:ablations_cont}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccc|ccc|ccc|ccc|ccc}
\toprule
 & \multirow{2}{*}{\textbf{\# Param}} & \multirow{2}{*}{\textbf{Deep}} & \multirow{2}{*}{\textbf{No Grad}} & \multicolumn{3}{c|}{SFoV} & \multicolumn{3}{c|}{SFoV+Dist} & \multicolumn{3}{c|}{LFoV} & \multicolumn{3}{c}{Pano} \\
 & & & & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_{5^{\circ}}}\uparrow$ & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_{5^{\circ}}}\uparrow$ & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_{5^{\circ}}}\uparrow$ & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_{5^{\circ}}}\uparrow$ \\
\midrule
1 & 1 & \cmark & \cmark & $-$ & $66.3$ & $-$ & $-$ & $39.2$ & $-$ & $-$ & $42.2$ & $-$ & $-$ & $6.0$ & $-$ \\
2 & 4 & \cmark & \cmark & $-$ & $64.3$ & $-$ & $-$ & $35.1$ & $-$ & $-$ & $47.9$ & $-$ & $-$ & $5.7$ & $-$ \\
3 & 3 & \cmark & \xmark & $-$ & $67.5$ & $-$ & $-$ & $52.1$ & $-$ & $-$ & $44.8$ & $-$ & $-$ & $6.4$ & $-$ \\
4 & 3 & \xmark & \cmark & $-$ & $65.8$ & $-$ & $-$ & $58.0$ & $-$ & $-$ & $47.6$ & $-$ & $-$ & $6.9$ & $-$ \\
5 & 3 & \cmark & \cmark & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> tables/atomic_old/adt_k360.tex <==
\begin{table}
\centering
\caption{\textbf{Comparison on zero-shot evaluation for ScanNet++~DSLR and KITTI360.} Missing values (\textcolor{gray}{-}) indicate the model's inability to produce the respective output. \dag: ground-truth camera for 3D reconstruction. \ddag: ground-truth camera for 2D depth map inference.}
\vspace{-10pt}
\label{tab:supp:atomic_adtk360}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccc|ccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}}  & \multicolumn{3}{c|}{ADT} & \multicolumn{3}{c}{KITTI360} \\
     & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ \\
    \midrule
    DepthAnything~\cite{yang2024da1} & $81.7$ & \textcolor{gray}{-} & \textcolor{gray}{-} & $9.5$ & \textcolor{gray}{-} & \textcolor{gray}{-} \\
    DepthAnythingv2~\cite{yang2024da2} & $82.6$ & \textcolor{gray}{-} & \textcolor{gray}{-} & $11.3$ & \textcolor{gray}{-} & \textcolor{gray}{-} \\
    Metric3D\textsuperscript{\dag \ddag}~\cite{yin2023metric3d} & $85.3$ & $65.4$ & \textcolor{gray}{-} & $39.7$ & $0.2$ & \textcolor{gray}{-} \\
    Metric3Dv2\textsuperscript{\dag \ddag}~\cite{hu2024metric3dv2} & $92.4$ & $67.3$ & \textcolor{gray}{-} & $43.9$ & $0.1$ & \textcolor{gray}{-} \\
    ZoeDepth\textsuperscript{\dag}~\cite{bhat2023zoedepth} & $83.5$ & $15.3$ & \textcolor{gray}{-} & $41.2$ & $0.2$ & \textcolor{gray}{-} \\
    UniDepth~\cite{piccinelli2024unidepth} & $90.8$ & $27.1$ & $32.1$ & $44.0$ & $14.6$ & $7.1$ \\
    MASt3R~\cite{leroy2024master} & $86.7$ & $52.5$ & $51.4$ & $41.7$ & $15.7$ & $7.4$ \\
    DepthPro~\cite{bochkovskii2024depthpro} & $81.3$ & $47.9$ & $48.0$ & $38.0$ & $5.9$ & $17.5$ \\
    \midrule
    \ourmodel-Small & $93.7$ & $83.3$ & $92.0$ & $\scnd{81.7}$ & $59.5$ & $\scnd{82.6}$ \\
    \ourmodel-Base & $\scnd{94.8}$ & $\scnd{88.1}$ & $\scnd{93.7}$ & $80.7$ & $\scnd{61.2}$ & $80.8$ \\
    \ourmodel-Large & $\best{95.5}$ & $\best{89.3}$ & $\best{93.9}$ & $\best{85.4}$ & $\best{65.6}$ & $\best{83.2}$ \\
    \bottomrule
\end{tabular}%
}
\end{table}

==> tables/atomic_old/diof_spp.tex <==
\begin{table}
\centering
\caption{\textbf{Comparison on zero-shot evaluation for Diode (Indoor) with distortion and ScanNet++~DSLR.} Missing values (\textcolor{gray}{-}) indicate the model's inability to produce the respective output. \dag: ground-truth camera for 3D reconstruction. \ddag: ground-truth camera for 2D depth map inference.}
\vspace{-10pt}
\label{tab:supp:atomic_diofspp}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccc|ccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}}  & \multicolumn{3}{c|}{DiodeIndoor\textsubscript{F}} & \multicolumn{3}{c}{ScanNet++~(DSLR)} \\
     & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ \\
    \midrule
    DepthAnything~\cite{yang2024da1} & $94.2$ & \textcolor{gray}{-} & \textcolor{gray}{-} & $51.4$ & \textcolor{gray}{-} & \textcolor{gray}{-} \\
    DepthAnythingv2~\cite{yang2024da2} & $89.3$ & \textcolor{gray}{-} & \textcolor{gray}{-} & $52.3$ & \textcolor{gray}{-} & \textcolor{gray}{-} \\
    Metric3D\textsuperscript{\dag \ddag}~\cite{yin2023metric3d} & $89.7$ & $26.5$ & \textcolor{gray}{-} & $51.2$ & $12.5$ & \textcolor{gray}{-} \\
    Metric3Dv2\textsuperscript{\dag \ddag}~\cite{hu2024metric3dv2} & $91.6$ & $35.8$ & \textcolor{gray}{-} & $71.3$ & $6.6$ & \textcolor{gray}{-} \\
    ZoeDepth\textsuperscript{\dag}~\cite{bhat2023zoedepth} & $90.1$ & $35.5$ & \textcolor{gray}{-} & $71.2$ & $3.6$ & \textcolor{gray}{-} \\
    UniDepth~\cite{piccinelli2024unidepth} & $94.7$ & $\scnd{37.2}$ & $74.8$ & $71.0$ & $9.1$ & $20.2$ \\
    MASt3R~\cite{leroy2024master} & $89.3$ & $29.5$ & $83.0$ & $73.0$ & $21.0$ & $16.6$ \\
    DepthPro~\cite{bochkovskii2024depthpro} & $86.0$ & $26.5$ & $75.7$ & $74.1$ & $24.4$ & $30.9$ \\
    \midrule
    \ourmodel-Small & $95.0$ & $33.0$ & $82.2$ & $78.2$ & $23.7$ & $35.6$ \\
    \ourmodel-Base & $\scnd{96.2}$ & $\best{37.2}$ & $\scnd{85.3}$ & $\scnd{86.5}$ & $\scnd{53.8}$ & $\scnd{65.1}$ \\
    \ourmodel-Large & $\best{97.7}$ & $36.0$ & $\best{86.4}$ & $\best{92.7}$ & $\best{59.9}$ & $\best{68.6}$ \\
    \bottomrule
\end{tabular}%
}
\end{table}

==> tables/atomic_old/eth_ibims.tex <==
\begin{table}
\centering
\caption{\textbf{Comparison on zero-shot evaluation for ETH3D and IBims-1.} Missing values (\textcolor{gray}{-}) indicate the model's inability to produce the respective output. \dag: ground-truth camera for 3D reconstruction. \ddag: ground-truth camera for 2D depth map inference.}
\vspace{-10pt}
\label{tab:supp:atomic_ethibims}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccc|ccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}}  & \multicolumn{3}{c|}{ETH3D} & \multicolumn{3}{c}{IBims} \\
     & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ \\
    \midrule
    DepthAnything~\cite{yang2024da1} & $93.2$ & \textcolor{gray}{-} & \textcolor{gray}{-} & $97.0$ & \textcolor{gray}{-} & \textcolor{gray}{-} \\
    DepthAnythingv2~\cite{yang2024da2} & $93.3$ & \textcolor{gray}{-} & \textcolor{gray}{-} & $98.0$ & \textcolor{gray}{-} & \textcolor{gray}{-} \\
    Metric3D\textsuperscript{\dag \ddag}~\cite{yin2023metric3d} & $81.1$ & $19.9$ & \textcolor{gray}{-} & $96.2$ & $62.4$ & \textcolor{gray}{-} \\
    Metric3Dv2\textsuperscript{\dag \ddag}~\cite{hu2024metric3dv2} & $89.7$ & $\best{69.8}$ & \textcolor{gray}{-} & $\best{98.8}$ & $54.6$ & \textcolor{gray}{-} \\
    ZoeDepth\textsuperscript{\dag}~\cite{bhat2023zoedepth} & $86.1$ & $31.5$ & \textcolor{gray}{-} & $95.8$ & $53.5$ & \textcolor{gray}{-} \\
    UniDepth~\cite{piccinelli2024unidepth} & $93.9$ & $27.6$ & $42.6$ & $98.1$ & $30.3$ & $\best{76.6}$ \\
    MASt3R~\cite{leroy2024master} & $91.3$ & $28.4$ & $\best{92.2}$ & $95.1$ & $55.7$ & $\scnd{76.0}$ \\
    DepthPro~\cite{bochkovskii2024depthpro} & $81.1$ & $41.2$ & $77.4$ & $98.0$ & $62.8$ & $75.9$ \\
    \midrule
    \ourmodel-Small & $94.2$ & $44.3$ & $80.8$ & $97.7$ & $67.3$ & $74.4$ \\
    \ourmodel-Base & $\scnd{95.8}$ & $53.8$ & $82.1$ & $98.0$ & $\scnd{67.5}$ & $73.3$ \\
    \ourmodel-Large & $\best{96.4}$ & $\scnd{56.7}$ & $\scnd{88.2}$ & $\scnd{98.7}$ & $\best{71.5}$ & $75.4$ \\
    \bottomrule
\end{tabular}%
}
\end{table}


==> tables/atomic_old/ethf_ibimsf.tex <==
\begin{table}
\centering
\caption{\textbf{Comparison on zero-shot evaluation for ETH3D and IBims-1 with distortions.} Missing values (\textcolor{gray}{-}) indicate the model's inability to produce the respective output. \dag: ground-truth camera for 3D reconstruction. \ddag: ground-truth camera for 2D depth map inference.}
\vspace{-10pt}
\label{tab:supp:atomic_ethfibimsf}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccc|ccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}}  & \multicolumn{3}{c|}{ETH3D\textsubscript{F}} & \multicolumn{3}{c}{IBims\textsubscript{F}} \\
     & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ \\
    \midrule
    DepthAnything~\cite{yang2024da1} & $91.8$ & \textcolor{gray}{-} & \textcolor{gray}{-} & $97.1$ & \textcolor{gray}{-} & \textcolor{gray}{-} \\
    DepthAnythingv2~\cite{yang2024da2} & $83.9$ & \textcolor{gray}{-} & \textcolor{gray}{-} & $93.4$ & \textcolor{gray}{-} & \textcolor{gray}{-} \\
    Metric3D\textsuperscript{\dag \ddag}~\cite{yin2023metric3d} & $80.9$ & $27.0$ & \textcolor{gray}{-} & $93.3$ & $56.6$ & \textcolor{gray}{-} \\
    Metric3Dv2\textsuperscript{\dag \ddag}~\cite{hu2024metric3dv2} & $83.5$ & $45.0$ & \textcolor{gray}{-} & $93.3$ & $60.6$ & \textcolor{gray}{-} \\
    ZoeDepth\textsuperscript{\dag}~\cite{bhat2023zoedepth} & $86.1$ & $36.8$ & \textcolor{gray}{-} & $94.5$ & $48.1$ & \textcolor{gray}{-} \\
    UniDepth~\cite{piccinelli2024unidepth} & $90.1$ & $38.5$ & $67.5$ & $97.2$ & $53.3$ & $69.3$ \\
    MASt3R~\cite{leroy2024master} & $87.7$ & $32.0$ & $\best{78.5}$ & $92.8$ & $44.1$ & $69.7$ \\
    DepthPro~\cite{bochkovskii2024depthpro} & $72.7$ & $29.1$ & $69.9$ & $83.0$ & $32.4$ & $69.5$ \\
    \midrule
    \ourmodel-Small & $92.9$ & $49.9$ & $68.1$ & $97.6$ & $\scnd{62.3}$ & $71.0$ \\
    \ourmodel-Base & $\scnd{95.1}$ & $\scnd{53.6}$ & $67.3$ & $\scnd{98.3}$ & $59.7$ & $\scnd{72.6}$ \\
    \ourmodel-Large & $\best{95.6}$ & $\best{60.4}$ & $\scnd{73.1}$ & $\best{98.6}$ & $\best{67.2}$ & $\best{76.9}$ \\
    \bottomrule
\end{tabular}%
}
\end{table}

==> tables/atomic_old/nu_dio.tex <==
\begin{table}
\centering
\caption{\textbf{Comparison on zero-shot evaluation for NuScenes and Diode (Indoor).} Missing values (\textcolor{gray}{-}) indicate the model's inability to produce the respective output. \dag: ground-truth camera for 3D reconstruction. \ddag: ground-truth camera for 2D depth map inference.}
\vspace{-10pt}
\label{tab:supp:atomic_nudio}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccc|ccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}}  & \multicolumn{3}{c|}{Nuscenes} & \multicolumn{3}{c}{DiodeIndoor} \\
     & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ \\
    \midrule
    DepthAnything~\cite{yang2024da1} & $79.0$ & \textcolor{gray}{-} & \textcolor{gray}{-} & $97.5$ & \textcolor{gray}{-} & \textcolor{gray}{-} \\
    DepthAnythingv2~\cite{yang2024da2} & $79.4$ & \textcolor{gray}{-} & \textcolor{gray}{-} & $97.6$ & \textcolor{gray}{-} & \textcolor{gray}{-} \\
    Metric3D\textsuperscript{\dag \ddag}~\cite{yin2023metric3d} & $64.0$ & $57.4$ & \textcolor{gray}{-} & $91.3$ & $38.2$ & \textcolor{gray}{-} \\
    Metric3Dv2\textsuperscript{\dag \ddag}~\cite{hu2024metric3dv2} & $64.8$ & $64.0$ & \textcolor{gray}{-} & $\best{98.5}$ & $\best{71.8}$ & \textcolor{gray}{-} \\
    ZoeDepth\textsuperscript{\dag}~\cite{bhat2023zoedepth} & $64.8$ & $29.7$ & \textcolor{gray}{-} & $91.8$ & $43.7$ & \textcolor{gray}{-} \\
    UniDepth~\cite{piccinelli2024unidepth} & $83.1$ & $64.4$ & $97.7$ & $97.2$ & $\scnd{63.0}$ & $\best{96.1}$ \\
    MASt3R~\cite{leroy2024master} & $63.5$ & $13.6$ & $78.3$ & $92.3$ & $48.8$ & $70.2$ \\
    DepthPro~\cite{bochkovskii2024depthpro} & $59.1$ & $46.5$ & $79.1$ & $93.9$ & $50.3$ & $71.5$ \\
    \midrule
    \ourmodel-Small & $83.8$ & $59.5$ & $96.0$ & $96.1$ & $49.2$ & $92.9$ \\
    \ourmodel-Base & $\scnd{86.7}$ & $\scnd{65.6}$ & $\scnd{97.9}$ & $97.4$ & $50.3$ & $91.1$ \\
    \ourmodel-Large & $\best{87.8}$ & $\best{68.5}$ & $\best{98.6}$ & $\scnd{97.8}$ & $48.9$ & $\scnd{93.3}$ \\
    \bottomrule
\end{tabular}%
}
\end{table}



==> tables/atomic_old/nyu_kit.tex <==
\begin{table}
\centering
\caption{\textbf{Comparison on zero-shot evaluation for NYUv2 and KITTI.} Missing values (\textcolor{gray}{-}) indicate the model's inability to produce the respective output. \dag: ground-truth camera for 3D reconstruction. \ddag: ground-truth camera for 2D depth map inference. *: trained on NYU and KITTI.}
\vspace{-10pt}
\label{tab:supp:atomic_nyukitti}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccc|ccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}}  & \multicolumn{3}{c|}{NYU} & \multicolumn{3}{c}{KITTI} \\
     & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ & $\mathrm{\delta_1^{SSI}}\uparrow$ & $\mathrm{F_A}\uparrow$ & $\mathrm{\rho_A}\uparrow$ \\
    \midrule
    DepthAnything~\cite{yang2024da1} & $97.8$ & \textcolor{gray}{-} & \textcolor{gray}{-} & $88.5$ & \textcolor{gray}{-} & \textcolor{gray}{-} \\
    DepthAnythingv2~\cite{yang2024da2} & $97.7$ & \textcolor{gray}{-} & \textcolor{gray}{-} & $88.4$ & \textcolor{gray}{-} & \textcolor{gray}{-} \\
    Metric3D\textsuperscript{\dag \ddag}~\cite{yin2023metric3d} & $89.0$ & $55.0$ & \textcolor{gray}{-} & $97.0$ & $25.4$ & \textcolor{gray}{-} \\
    Metric3Dv2\textsuperscript{\dag \ddag}~\cite{hu2024metric3dv2} & $98.1$ & $72.4$ & \textcolor{gray}{-} & $96.7$ & $25.5$ & \textcolor{gray}{-} \\
    ZoeDepth\textsuperscript{\dag}~\cite{bhat2023zoedepth} & $98.0$ & $78.9$ & \textcolor{gray}{-} & $96.7$ & $\scnd{82.6}$ & \textcolor{gray}{-} \\
    UniDepth~\cite{piccinelli2024unidepth} & $\best{99.0}$ & $\best{83.1}$ & $\best{99.2}$ & $\best{98.3}$ & $\best{85.8}$ & $\best{97.5}$ \\
    MASt3R~\cite{leroy2024master} & $94.8$ & $69.6$ & $90.7$ & $90.9$ & $10.9$ & $77.7$ \\
    DepthPro~\cite{bochkovskii2024depthpro} & $97.2$ & $73.0$ & $\scnd{93.1}$ & $94.8$ & $62.4$ & $80.9$ \\
    \midrule
    \ourmodel-Small & $97.4$ & $69.8$ & $84.0$ & $96.4$ & $77.8$ & $85.8$ \\
    \ourmodel-Base & $97.9$ & $75.5$ & $89.1$ & $97.3$ & $76.6$ & $82.7$ \\
    \ourmodel-Large & $\scnd{98.3}$ & $\scnd{81.4}$ & $90.9$ & $\scnd{97.7}$ & $81.4$ & $\scnd{90.3}$ \\
    \bottomrule
\end{tabular}%
}
\end{table}
